DUETS: A Dataset of Reproducible Pairs ofJava Library-Clients

Software engineering researchers look for software artifacts to study their characteristics or to evaluate new techniques. In this paper, we introduce DUETS, a new dataset of software libraries and their clients. This dataset can be exploited to gain many different insights, such as API usage, usage inputs, or novel observations about the test suites of clients and libraries. DUETS is meant to support both static and dynamic analysis. This means that the libraries and the clients compile correctly, they are executable and their test suites pass. The dataset is composed of open-source projects that have more than five stars on GitHub. The final dataset contains 395 libraries and 2,874 clients. Additionally, we provide the raw data that we use to create this dataset, such as 34,560 pom.xml files or the complete file list from 34,560 projects. This dataset can be used to study how libraries are used by their clients or as a list of software projects that successfully build. The client's test suite can be used as an additional verification step for code transformation techniques that modify the libraries.

==> figures/json_figure.tex <==
\begin{figure}
    \centering
    \begin{lstlisting}[language=json,firstnumber=1]
{
  "com.alibaba:fastjson": {
    "groupId": "com.alibaba",
    "artifactId": "fastjson",
    "repo_name": "alibaba/fastjson",
    "clients": {
      "1.2.46": [
        {
          "repo_name": "861763765/mqtt-demo",
          "groupId": "com.example.mqtt.demo", 
          "artifactId": "mqtt-demo",
          "version": "1.2.46",
          "commit": "4e704644e",
          "test_results": [
            { "error": 0, "failing": 0, "passing": 1, "execution_time": 0.525 },
            { "error": 0, "failing": 0, "passing": 1, "execution_time": 0.514 },
            { "error": 0, "failing": 0, "passing": 1, "execution_time": 0.75 }
          ]
        },
        ... // clients for the other releases
      ]
    },
    "releases": {
      "1.2.46": "00bbb28bf0",
      ... // commit sha for the other releases
    },
    "test_results": {
      "1.2.46": [
        {"passing": 4229, "failing": 0, "error": 0, "execution_time": 62.698},
        {"passing": 4229, "failing": 0, "error": 0, "execution_time": 62.755},
        {"passing": 4229, "failing": 0, "error": 0, "execution_time": 64.971}
      ],
      ... // test results for the other releases
    }
  },
  ... // other libraries
}
\end{lstlisting}
    \caption{Representation of the dataset in JSON format}
    \label{fig:dataset}
\end{figure}
